A Proposal for Foley Sound Synthesis Challenge

"Foley" refers to sound effects that are added to multimedia during post-production to enhance its perceived acoustic properties, e.g., by simulating the sounds of footsteps, ambient environmental sounds, or visible objects on the screen. While foley is traditionally produced by foley artists, there is increasing interest in automatic or machine-assisted techniques building upon recent advances in sound synthesis and generative models. To foster more participation in this growing research area, we propose a challenge for automatic foley synthesis. Through case studies on successful previous challenges in audio and machine learning, we set the goals of the proposed challenge: rigorous, unified, and efficient evaluation of different foley synthesis systems, with an overarching goal of drawing active participation from the research community. We outline the details and design considerations of a foley sound synthesis challenge, including task definition, dataset requirements, and evaluation criteria.

==> 2_first_paragraphs.tex <==
In this section, we review five existing research challenges: Blizzard Challenge, CHiME, DCASE, Music Demixing challenge, and AI Song Contest. The former three are relatively mature while the last two started after 2020. These challenges are based on various datasets and evaluation procedures adapted for their problem definitions. All of them started along with increasing popularity of the research problems and have contributed to the continued growth. % by providing reliable and accurate benchmarks. 


The Music Information Retrieval Evaluation eXchange (MIREX) was proposed in 2003 \cite{downie2003toward} and started in 2005 as a part of ISMIR~2005. There were 10 music information retrieval tasks such as genre identification and tempo extraction. In MIREX, participants usually submit their algorithms to a system for automatic evaluation on undisclosed datasets. Sometimes human evaluation was added due to the subjectivity of the tasks~\cite{downie2006music}, for example, audio music similarity and symbolic melodic similarity in 2006. MIREX has been popular among music researchers, becoming an important showcase of growing music information retrieval technologies.   % Unfortunately, MIREX has lost its popularity in the recent years with most of the tasks was discontinued in MIREX 2021. [why? ] % The recent paradigm changes in music information retrieval towards deep learning and..

==> 3_1_short.tex <==
\subsection{Previous Works on FSS}
  There are few works for AI-generated foley sound. It is not a new field that has never been researched. There are some papers on the topic of generating foot step based in physical modeling and signal processing[ref, ref, ref, ref]. Deep learning field has matured enough, but foley generation by AI still needs more studies.
 In [stick], they generated hitting and scratching stick sound using video dataset[The greatest Hits]. Following this work, some papers[AutoFoley, Towards, FoleyGAN, Taming] that make more general foley sound were released. They all generate foley sound based on the visual scene. Those models are capable of generating sound with precise time synchrosization and right class. As in those papers, all of the works are rely on visual sequence cues because they has very large and well-organized video datasets from youtube[ref, ref, ref].
 Therefore, audio-vision representation learning from video is beneficial for generating audio just like text-image generation such as [CLIP, DALL-E2]. In [AudioClip], three modalities - text, video, and audio are combined using pre-trained CLIP, and these encoders are then utilzed subtasks like retrieval, classification, etc. 
 To research foley generation, the time is now. Because have complete set- rich audio visual dataset, big progression in representation learning of audio and multi-modality, various and powerful generative models including auto-regressive[ref], VAE[ref], Flows[ref], GAN[ref], and finally Diffusion[DiffWave, SpecGrad]. Therefore generation of foley sound has room for improvement in short time.

==> 4_3_evaluation.tex <==
\subsection{Evaluation}

Evaluation of generative models or synthesized samples is a difficult task in general, and important particularly when organizing a challenge. 
Objective evaluation is convenient, but it often disagrees with the human perception. It may be also `gamed', which would be absolutely undesirable for a challenge.
% 
As an alternative, human-engaged evaluation has been widely used as a way of benchmark to compare performance for different audio generation models~\cite{hayashi2020espnet}.
% 
In practice, however, subjective evaluation may not be preferred in a large-scale evaluation due to the low time- and cost-efficiency. 


To combine advantages of objective and subjective evaluation, we suggest a two-phase evaluation scheme as follows:
\begin{itemize}
    \item
        \textbf{Phase 1}: All participants will be evaluated only with objective metrics. All metrics will be publicly announced and considered simultaneously in the public leader board.
        %
        % rank-based
        % The participated systems will be scored according to their rank for each metrics, and summation of this rank-based score is the final score for the first phase. 
        % With this rank-based evaluation scheme, various metrics can be accounted without selecting combination weight for each metric.
        %
        % normalize-and-sum
        The participating systems will be scored with respect to each objective metric. The scores will be standardized over all the evaluators, and the standardized scores will be summed to yield the final score of a system.
        % according to their \textit{standard scores} for each metrics. For balanced contribution of each metrics, all metrics will be standardized to have same average score and deviation.
        % With this evaluation scheme, various metrics can be accounted regardless of their statistics in original scales.
    \item
        \textbf{Phase 2}: Only the top-$N$ submissions from Phase 1 will be evaluated on 5-point scale (MOS). Human evaluators will be asked to focus on various aspects of the generated samples, e.g., fidelity, coincidence with class label, and temporal alignment. The final ranking will be decided by an average MOS.
\end{itemize}

In the following sections, we discuss the objective and subjective metrics to evaluate generative models.

\subsubsection{Objective Evaluation Metrics}
    In the first phase of the competition, inception score (IS) and Fréchet inception distance (FID) will be used to determine ranks of the participants. In order to detect severe memorization of training samples, which could happen as a result of overfitting, we will use the memorization-aware version of FID \cite{bai2021training} instead of the original FID. 
    
    \textbf{Inception score (IS)} % \cite{salimans2016improved}
    has gained popularity after its introduction to evaluate implicit generative models such as GANs. IS is defined with posterior distribution of auxiliary classifier models.
    % This can be interpreted as multiplication of sharpness $S$ and diversity $D$,
    % \begin{align*}
    %     IS = S \cdot D.
    % \end{align*}
    % For audio label $x$ and label $y$, the sharpness and diversity is defined as follows
    % \begin{align*}
    %     S &= \exp \big( \mathbb E_{\mathbf x\sim \mathcal G} [\int c(y|\mathbf x) \log c(y|\mathbf x) dy]) \\
    %     D &= \exp (-\mathbb E_{\mathbf x\sim \mathcal G} [\int c(y|\mathbf x) \log c(y) dy]),
    % \end{align*}
    % where $\mathcal G$ is the distribution of generated samples. Sharpness, in the above equation, represents how confident the classifier is to its output label. Diversity $D$, on the other hands, represents the class diversity of the generated samples.
    %
    IS is often interpreted as multiplication of sharpness and diversity, which represent the confidence of the classifier to its output label and the class diversity of the generated samples, respectively.
    In other words, IS is able to sensitively reflect the quality of class identity and diversity. However, it does not capture the mode inconsistency, i.e. mode addition or dropping. 
    
    
    \textbf{Fréchet inception distance (FID)} % \cite{heusel2017gans} 
    is another widely used metric for generative models. Instead of using \emph{outputs} of an auxiliary model as done in IS, the calculation of FID relies on \emph{hidden representations} of an auxiliary model. The auxiliary model does not need to be an classifier, and it is assumed that FID is robust to choice of representation space. Recently, FID was adopted for audio generation using an audio classifier and named Fréchet audio distance (FAD)~\cite{kilgour2019frechet}. 
    
    % FID or FAD is calculated from sets of hidden representation $\mathcal F_\mathcal G$ or $\mathcal F_\mathcal T$ for generated samples ($\mathcal G$) and real samples ($\mathcal T$) respectively.
    % Each set is fitted to multivariate Gaussian distribution extracting distribution parameter $(\mu, \Sigma)$. Then FID is obtained as,
    % \begin{align*}
    %     FID=\|\mu_\mathcal G - \mu_\mathcal T\|^2 
    %     + Tr(\Sigma_\mathcal G + \Sigma_\mathcal T - 2(\Sigma_\mathcal G\Sigma_\mathcal T)^{1/2}).
    % \end{align*}
    %
    FID (as well as FAD) is calculated from sets of hidden representations of generated and real samples. Each set of representation is fitted to a multivariate Gaussian distribution, and the Fréchet distance of these two distributions becomes the FID score of the generated samples.
    Since it directly models the distribution of hidden representations, FID is sensitive to mode changes including spurious mode addition or dropping \cite{sajjadi2018assessing}.
    
    % keunwoo: i'm commenting out Mi-FID. (lack of space)
    % % Mi-FID
    % In the first (and only to our best knowledge) challenge for deep generative modeling \footnote{https://www.kaggle.com/c/generative-dog-images}, memorization penalty is additionally considered upon FID metric \cite{bai2021training}. 
    % % Since the most widely adopted metrics, IS and FID are both prone to assign high score to the memorized samples from training set, intentional memorization must be properly penalized for fairness of the competition. 
    % Memorization-informed FID is the multiplication of FID and memorization penalty % $m_\tau$.
    % , which is an thresholded version of the following memory distance
    % % \begin{align*}
    % %     MiFID &= m_\tau \cdot FID
    % % \end{align*}
    % % \begin{align*}
    % %     m_\tau &= \begin{cases} 
    % %         \frac{1}{D(\mathcal G, \mathcal T) + \epsilon} ,     & \text{if}\, D(\mathcal G, \mathcal T) < \tau \\
    % %         1,                                                      & \text{otherwise}
    % %     \end{cases},
    % % \end{align*}
    % % where the memory distance is defined as 1 subtraction of cosine similarity as follows
    % \begin{align*}
    %     D(\mathcal G, \mathcal T) &= \frac{1}{|\mathcal G|} \sum_{\mathbf x \in \mathcal G} \bigg(
    %         1 - \frac{|\langle\mathbf x_\mathcal G \cdot \mathbf x_\mathcal T\rangle|}{|\mathbf x_\mathcal G|\cdot|\mathbf x_\mathcal T|}
    %     \bigg).
    % \end{align*}
    % The threshold for memorization penalty is determined empirically with two different goals; (i) enough distinguishability for intentional or severe memorization, and (ii) least change to the FID score as possible.
    
    % \textit{Bai et al.} \cite{bai2021training} also pointed out that FID is not robust enough to the latent space selection, i.e. the metric might differ a lot depending on the auxiliary model for feature projection. In order to avoid attempt which overfit to specific feature space, they used separate models for their public and private leaderboards.
    % Accepting the lesson from the challenge, we would consider to include detection and penalty for the memorization and would care the latent space selection for the scoring model for IS and FID.
    
    % \textbf{CaptionScore}
    
    
    % decided to comment out R-precision.
    % \textbf{R-Precision}
    % is a performance metric that is used in a ranking retrieval task. According to the definition, $R$ indicates the number of the query-related documents for a given query and a dataset. Among the top-$R$ retrieved documents by the system, the ratio of truly related documents 
    % % (hence, \textit{precision} in the name) 
    % is the R-precision of the system.
    % This metric was adopted for text-to-image generation task in~\cite{xu2018attngan} as follows. For each image sample, 100 text descriptions are ranked according to their cosine similarity in the feature space, and then its precision is calculated.
    % Among the text description, only one sample is ground truth, i.e. $R=1$, and the others are negative samples.
    % For text- or video-to-audio synthesis, this can be used to evaluate condition consistency using a pretrained multi-modal encoder.
    
    
\textbf{Likelihood} is worth discussing, although we do not recommend using it. It is
    one of the most straightforward metric for evaluation of generative models. For density estimation, likelihood is a key metric as it directly shows how the model estimates the target distribution. However, we suggest not using likelihood for two reasons. First, it is often not aligned with perceptual quality \cite{Theis2016a}. Second, it has limited applicability since calculation of likelihood is not possible for some generative models such as including GANs, VAEs or, diffusion probabilistic models. 
    
\subsubsection{Subjective Evaluation Metrics}
% Subjective evaluation is often used to evaluate generative models across various applications to focus on perceptual quality. % for diverse features can be directly assessed through human-engaged test. 
Perhaps the most common scheme of subjective evaluation is to ask the mean opinion score (MOS). In MOS test, human raters are guided to evaluate a sample into five-point scale where 1 means \emph{very bad} and 5 means \emph{very natural}. Usually, there are various aspects that affect the overall perceptual quality such as fidelity, degree of artifacts, and naturalness. To measure them separately, it is common to design multiple questions for each sample.
In the proposed challenge, we suggest the following criteria in the subjective evaluation.
\begin{itemize}
    \item Fidelity of generated audio
    \item Distortions and artifacts of generated audio
    \item Coincidence to the given conditions, e.g. class labels, text descriptions, or video frames
\end{itemize}
% We do not consider MUSHRA Test \cite{} to encourage raters with diverse backgrounds to participate the evaluation procedure.
